A Survey of Moving Target Defenses for Network Security

Network defenses based on traditional tools, techniques, and procedures fail to account for the attacker's inherent advantage present due to the static nature of network services and configurations. To take away this asymmetric advantage, Moving Target Defense (MTD) continuously shifts the configuration of the underlying system, in turn reducing the success rate of cyberattacks. In this survey, we analyze the recent advancements made in the development of MTDs and define categorizations that capture the key aspects of such defenses. We first categorize these defenses into different sub-classes depending on what they move, when they move and how they move. In trying to answer the latter question, we showcase the use of domain knowledge and game-theoretic modeling can help the defender come up with effective and efficient movement strategies. Second, to understand the practicality of these defense methods, we discuss how various MTDs have been implemented and find that networking technologies such as Software Defined Networking and Network Function Virtualization act as key enablers for implementing these dynamic defenses. We then briefly highlight MTD test-beds and case-studies to aid readers who want to examine or deploy existing MTD techniques. Third, our survey categorizes proposed MTDs based on the qualitative and quantitative metrics they utilize to evaluate their effectiveness in terms of security and performance. We use well-defined metrics such as risk analysis and performance costs for qualitative evaluation and metrics based on Confidentiality, Integrity, Availability (CIA), attack representation, QoS impact, and targeted threat models for quantitative evaluation. Finally, we show that our categorization of MTDs is effective in identifying novel research areas and highlight directions for future research.

==> sections/03_mtd_03_05_2020.tex <==

\section{Moving Target Defense Techniques}
\label{sec:mtd}

The goal of \emph{Moving Target Defense} (MTD) is to move the components of a system in a continuous and randomized fashion. This increases the uncertainty for the attacker, making it harder (or costlier) for them to successfully exploit the system. For example, the information gathered by the attacker in the \emph{reconnaissance phase} might become \emph{stale} during the \emph{attack phase} if the defender has moved to a new configuration in that time. Furthermore, we believe that MTD can be used as a meta-defense technique that can be used in conjunction with traditional defense methods to provide better security while ensuring the minimum impact on performance.

Let us now discuss the formalism of Markov Games~\cite{littman2001value}. This is a generalization of the formalism defined for MTDs in \cite{zhuang2014towards} and helps us capture the various aspects of the various MTDs surveyed.
An MTD system can be specified by the tuple $\langle S, A^\mathcal{D}, A^\mathcal{A}, T, R^\mathcal{D}, R^\mathcal{A} \rangle$ where $S$ denotes the state of the MTD system (or a deployed configuration), $A$ denotes the set of actions or pure strategies the defender ($A^\mathcal{D}$) or the attacker ($A^\mathcal{A}$) can take, $T: S\times A \rightarrow S$ represents a transition function over he joint space of actions (i.e. $A: A^\mathcal{D} \times A^\mathcal{A}$), and $R:T \rightarrow \mathbb{R}$ represents the reward/loss on performing a transition ($R^\mathcal{D}$) or an attack ($R^\mathcal{A}$). We will use the superscripts $\mathcal{D}$ and $\mathcal{A}$ to represent the functions for the defender and the attacker respectively.

Note that most of the elements in the tuple such as $S$ and $A^\mathcal{D}$ are highly problem-specific and can only be concretely defined in the context of a particular moving target defense. Although we do this later, we believe that an overview of how the different defenses model the various elements of the tuple help us to
(1) get a holistic view of the various MTD mechanisms, giving us a sense of what kind of modeling makes a particular defense more effectively, and (2) highlight opportunities on how modeling of a particular element can be improved or combined with other MTDs.



Having defined the formalism that we will use throughout the survey, we now describe our plan to categorize of the various MTDs. We ask three questions that are relevant for any moving target defense-- (1) \emph{what to switch?}, i.e. the kind of surface that is being shifted by the MTD system, (2) \emph{when to switch?}, i.e. finding an event after which a defender should shift, and (3) \emph{how to switch?}, i.e. finding a mechanism that, given the present state of the system, calculates a reasonable action to take. We then show how answers to these questions can help us in coming up with useful categorizations.

%\texthl{Incorporating the papers in the other two sections on implementation and evaluation into this section.}

\subsection{What to Switch? $\approx$ What actions to play?}

At a high level, every software system vulnerable to attacks can be defined to have four surfaces. These are:

\begin{itemize}
    \item Exploration Surface
    \item Attack Surface
    \item Detection Surface
    \item Prevention Surface
\end{itemize}

These surfaces interact with one another in complex ways, especially in the context of Advanced Persistent Threats (APT) (see Fig. \ref{fig:mtd-apt}). A strong adversary first tries to explore the target network, trying to figure out its topology, bandwidth, software deployed on the different nodes, etc. The exploration surface accounts for reconnaissance, verifying if it has actually gained access and established a foothold and a new vantage point to further explore the deployed system. All this knowledge helps an adversary to execute attacks that can exploit the system, helping them to move to different points in the network, gather and ex-filtrate important information.
As both exploration and attack traffic tend to be malicious in nature and thus, different from legitimate user traffic, the detection and prevention surface can come into play at any point in time.\\
%We now describe the works in context to the surface(s) they shift, followed by a discussion about works that shifts more than one surface and thus, falls at the intersection of two or more individual areas.
\indent In Fig. \ref{fig:what}, we show a Venn diagram that categorized existing MTDs based on what surfaces they shift. Although there exists overlap among the various research areas (especially when viewed from the perspective of APTs), most MTDs shift one surface at a time, hardly discussing what happens to the other surfaces. After discussing the various MTDs, we highlight some unexplored areas that can lead to development of new defense methods which shift multiple surfaces.

\begin{figure*}
\small
\centering
\begin{tikzpicture}
\begin{scope}[opacity=0.5]
    % everything is polar co-ordinates
    % (angle from origin [0-360], distance)
    \fill[Salmon!30!white,draw=black] (90:3) ellipse (4 and 3.5);
    \fill[SpringGreen!50!white,draw=black] (180:3.5) ellipse (5.55 and 3.9);
    \fill[Goldenrod!30!white,draw=black] (270:2.7) circle (2.7);
    \fill[CornflowerBlue!30!white,draw=black]  (360:4) circle (3.25 and 3);
    
 \end{scope}    
    % Exp Surface
    \node at (90:5.75) {\textbf{Exploration Surface Shifting(ES)}};
    \node at (106:5.45) {Al-Shaer et al.~\cite{al2012random}};
    \node at (109:5) {Albanese et al.~\cite{albanese2013moving}};
    \node at (116:4.7) {Jafarian et al.~\cite{jafarian2012openflow}};
    \node at (74:5.45) {Aydeger et al.~\cite{aydeger2016mitigating}};
    \node at (70:5) {Zhao et al.~\cite{zhao2017sdn}};
    \node at (66:4.58) {Schlenker et al.~\cite{schlenker2018deceiving}};
    \node at (60:4.15) {Jajodia et al.~\cite{jajodia2018share}};
    \node at (60:3.5) {Algin et al.~\cite{algin2017mitigating}};
     
    % Attack + Exp Surface
    \node at (130:4.2) {\textbf{AS+ES}};
    \node at (131:3.6) {Lei et al.~\cite{lei2017optimal}};
    \node at (132:3.1) {Zhuang et al.~\cite{zhuang2014towards}};
   
    % Attack Surface
    \node at (159:6.3) {\textbf{Attack Surface Shifting(AS)}};
    \node at (164:6.3) {Manadhata et al.~\cite{manadhata2013game}};
    \node at (168:6.3) {Zhu et al.~\cite{zhu2013game}};
    \node at (172:6.3) {Sengupta et al.~\cite{sengupta2017game}};
    \node at (176:6.3) {Carter et al.~\cite{carter2014game}};
    \node at (180:6.3) {Thompson et al.~\cite{thompson2014multiple}};
    \node at (184:6.3) {Chowdhary et al.~\cite{chowdhary2016sdn}};
    \node at (188:6.3) {El Mir et al.~\cite{el2016softwarel}};
    \node at (192:6.3) {Debroy et al.~\cite{debroy2016frequency}};
    \node at (196:6.3) {Prakash et al.~\cite{prakash2015empirical}};
    \node at (200:6.3) {Neti et al.~\cite{neti2012software}};
    \node at (204:6.3) {Crouse et al.~\cite{crouse2012improving}};
    \node at (208:6.3) {Bohara et al.~\cite{bohara2017moving}};
    
    % Prevention Surface
    \node at (270:4)    {\textbf{Prevention Surface Shifting(PS)}};
    \node at (270:4.45)    {Chowdhary et al.~\cite{chowdhary2017dynamic}};
    \node at (270:4.85)    {Clark et al.~\cite{clark2015game}};
  
    % Detection Surface Shifting
    \node at (350:5.1) {Colbaugh et al.~\cite{colbaugh2012predictability}};
    \node at (360:5.15) {Venkatesan et al.~\cite{venkatesan2016moving}};
    \node at (355:5.15) {Sengupta et al.~\cite{sengupta2018moving,senguptageneral}};
    \node at (345:5.15) {Chowdhary et al.~\cite{chowdhary2018markov}};
    \node at (5:5.15)    {\textbf{Detection Surface Shifting(DS)}};
  
  %\node [font=\Large] {\LaTeX};
  \end{tikzpicture}
    
%\end{comment}

\caption{The different surfaces that can be moved by a particular Moving Target Defense (MTD). Moving the exploration surface makes it harder for the attacker to figure out the exact system configuration by making the sensing actions noisy or untrue. Moving the attack surface makes a particular attack inapplicable. Moving the detection surface, similar to `patrolling methods', helps in providing efficient detection in budget-constrained cyber environments. Moving the prevention surface makes it harder for an attacker to ex-flitrate data even when they have a strong foot-hold insider the system.}
\label{fig:what}
\vspace{-1.6em}
\end{figure*}


\subsubsection{\textbf{Exploration Surface Shifting}}\label{exp}

The main motivation behind shifting the exploration surface is to ensure that the information an attacker can gather by scanning for open-ports, sending non-malicious traffic to uncover system topology, discover vulnerabilities, etc. is noisy or inaccurate. Thus, an adversary, with this faulty information from the reconnaissance, will have to shoot arrows (attacks) in the blind.

In \cite{al2012random,albanese2013moving}, the authors propose the concept of Random Host Mutation (RHM)-- moving target hosts are assigned random virtual IP addresses (vIP) in an unpredictable and distributed way. Formally, the action space $A^\mathcal{D}$ of configurations is the set of mappings from the set of vIP addresses in the Virtual Address Range (VAR) to the set of hosts in the network. Each action $\in A^\mathcal{D}$ represents a particular one-to-one mapping in a bipartite graph that consists a set of VARs and a set of hosts. Another work \cite{jafarian2012openflow} try to implement the same defense methods using a centralized approach that uses \emph{(SDN)} technologies like \emph{OpenFlow}.


% In \cite{jafarian2012openflow}, the authors seek to implement the same defense method using a centralized approach that uses \emph{software-defined networking} (SDN) technologies like \emph{OpenFlow}.

Another line of work tries to reduce the quality of information an attacker can retrieve through exploration. In \cite{aydeger2016mitigating}, the authors use a centralized approach to obfuscate the network links so that the topology that an attacker can retrieve via crossfire attacks is noisy and unreliable. In this work, each state is a possible path from the source to the destination of the crossfire attack. Thus, the action space, i.e. the set of defender configurations, $A^\mathcal{D}$ is the set of all paths from a source point to a destination point in the network under attack. The MTD paradigm comes into play because the administrator chooses one path, in a randomized fashion, so that the attacker is not able to get a piece of reliable and deterministic path information between the two points in the network. They are thus forced to use a lot of attack traffic in order to retrieve a good topology of the underlying network, thereby increasing their chances of getting caught or having to deal with an inaccurate (hopefully, not useful) topology. On similar lines, there have been works that either try to move the fingerprint of a protected host \cite{zhao2017sdn} or randomly alter the time schedule that guides when a host transmits, reducing the effectiveness against selective jamming attacks against smart meters \cite{algin2017mitigating}. In \cite{schlenker2018deceiving}, the authors propose to send back incorrect information to an attacker trying to query information about the hosts on the network. Although they come up with deterministic strategies for responses, the possibility of sending back different lies about the underlying system opens up the possibility for an MTD solution for shifting the exploration surface. These works are termed as {\em cyber-deception} because the defender is trying to deceive the adversary by feeding them false information about the system. In such cases, the goal of the defender is to ensure that the adversaries model of the underlying network is incorrect as opposed to simply incomplete or noisy.

In \cite{jajodia2018share}, Jajodia et al. looks at how they can deploy \emph{honey-nets} in a strategic fashion. They show that deploying honey-nets introduce deception in the network against \emph{noisy-rich} (NR) cyber-attackers (i.e. adversaries who try to exploit all the vulnerabilities present in order to compromise the target network). In this case, if we can represent the set of honey-nets by $H$, then the action space $A^\mathcal{D}$ of configuration consists of all the subsets of honey-nets. Each state $a \in A^\mathcal{D}$, which is a subset of $H$ ($a \subset H$) that are currently deployed.

\subsubsection{\textbf{Attack Surface Shifting}}\label{att}

Most of the work from the research community, both in cyber-security and in artificial intelligence, has focused on this area. The main aim of switching between attack surfaces is to render an attack action, that the attacker chooses after some exportation, \emph{invalid} (for example, an attack to exploit a \emph{Linux-based OS} will be useless if it is run on a machine running a \emph{Windows OS}. We first discuss some MTD methods that are defined at an abstract level to be applicable to various parts of a network environment and then, focus on more specific ones.

In one of the earlier works \cite{manadhata2013game}, the authors have a set of systems, which forms their space of MTD configurations, and each configuration $a \in A^\mathcal{D}$ can be represented by an attack surface characterized by three properties-- (1) the set of entry and exit points into the system, (2) the set of \emph{channels} and (3) the set of untrusted items (data/system/network link) in the particular state $a$. The aim of the defender is to switch between the different states (or systems) so as to maximize the shifting of the attack surface and at the same time, have minimum impact on performance. This multi-objective trade-off is a common theme in most of the other works as well.

In \cite{zhu2013game}, Zhu and Bashar break down a full-stack system into a number of layers (denoted by $l$). For each layer, they have a set of technologies that can be used to provide the functionality that the layer is responsible for. Now, when all layers (or stacks) come together to form the full-stack system, all possible combination of technologies cannot be used to provide proper functionality to the end user. Thus, from all these possible combinations, they handpick a few technologies that meet the use-case demands for the full-stack software among which they switch. Thus, this represents the defender's action space $A^\mathcal{D}$ for their system.
On similar lines, Sengupta et al. \cite{sengupta2017game} also assumes a full-stack web-application and thus, similar action sets where the technologies relate to web-stack development. The two papers differ in the way they decide {\em how to switch}, which we shall discuss in detail later.

Carter et al. in \cite{carter2014game}, designs an MTD system that switches between different Operating Systems (OSs) (they call these `platforms'). Thus, in their case, the defender's action set $A^\mathcal{D}$ is a set of all OSs that they can move between and $a \in A^\mathcal{D}$ is a single operating system. They also mention a notion of similarity (or diversity) between two systems in $A^\mathcal{D}$ on the basis of code structure and logic. Authors in \cite{thompson2014multiple} move away from MTD techniques that are abstract and expected to work in general for all cyber systems. They implement an MTD that can perform the OS rotation for machines deployed in the underlying network using a centralized mechanism. We now shift our attention to MTDs that move elements solely relating to networks.

In \cite{chowdhary2016sdn}, Chowdhary et al. describes an MTD that leverages port hoping to thwart exploits of known attack on a cloud-based system. In their work, the states of the system are composed of variables, each of which indicates if a certain vulnerability in the system has been exploited (or not) and based on it, decides when and how to move. This fits well with our discussion as to how attack surface shifting may happen after the detection surface comes into play. Along similar lines, authors in \cite{el2016softwarel} move a deployed VM to a different physical server if the impact of known vulnerabilities (measured using particular metrics) on the physical server exceeds a threshold. In \cite{debroy2016frequency}, the authors implement MTD at a different level where they move the services deployed on a particular VM to another VM. A natural extension could be to use both the layers for designing a hybrid MTD that shifts both services between the VMs and the VMs between the actual physical servers in the cloud network resulting in a multi-layer MTD, as discussed before \cite{sengupta2017game,zhu2013game}.

In \cite{prakash2015empirical}, authors talk about a range of configurations (precisely $72$ of them) and analyze the effect of using various game-theoretic strategies for switching between them. They shed some light on the amount of security gain that can be achieved in various settings. In \cite{neti2012software}, the authors point out a fundamental assumption that is often inherent in cybersecurity in general and MTD systems in particular-- the different configurations of the MTD are not vulnerable to the same attack (similar to the notion of diversity described in \cite{carter2014game}). They create a bipartite graph that maps hosts to vulnerabilities and show that MTD is more effective when the diversity is higher. This result is in lines with work in the security of Deep Neural Networks (DNN) where higher differential immunity to attacks leads to higher gains in robustness for ensembles based on MTD \cite{sengupta2018mtdeep}.

In rare cases, the number of playable actions in $A^\mathcal{D}$ may become huge. Due to computation and implementation challenges, a solution could be to first reduce $A^\mathcal{D}$ to $\hat{A}^\mathcal{D}$ such that $|\hat{A}^\mathcal{D}| \ll |A^\mathcal{D}|$ and then, implement an MTD with $A^\mathcal{D}=\hat{A}^\mathcal{D}$. In \cite{crouse2012improving}, researchers solve the first problem of finding a diverse $S'$ using a \textit{genetic algorithm} search methods. 
On the other hand, authors in \cite{bohara2017moving} showcase an MTD system that moves between containers and highlight that migration between containers, i.e., transition costs between the different states hardly results in a performance drop. Unfortunately, they are not able to generalize that such guarantees will hold for all MTD methods.

\subsubsection{\textbf{Detection Surface Shifting}}\label{dec}

The concept of detecting attacks from traffic on the wire or behavior or a request on a host machine has been a cornerstone of cybersecurity. Unfortunately, placing all possible Intrusion Detection Systems (IDS) on a system, especially in the case of large network leads to a degradation in the performance of the system. Thus, to minimize the impact of performance while keeping the attacker guessing about whether their attack will be detected or not, researchers have looked at intelligent ways in which a limited number of detection systems can be placed in the underlying network. These methods are similar to patrolling methods that try to identify security violation in physical security domains like airports, wildlife sanctuaries, etc. \cite{sinha2015physical}.

In \cite{venkatesan2016moving} and \cite{sengupta2018moving}, authors show that when faced with stealthy botnets or external adversaries who are powerful enough to attack any internal node of a deployed system, shifting the detection surface helps to maintain system performance, while being effective in detecting an ongoing attack.  In both of these cases, they have a set of nodes $N$ that is deployed in the network. The action set of the defender is composed of all $k$-sized subsets of $N$, i.e., $A^\mathcal{D}=\{N_k : N_k \subset N \cap |N_k| = k (< |N|)\}$. In \cite{chowdhary2018markov}, the authors argue that in many real-world multi-layered networks. The author's assumption of an attacker being able to attack from any point is too strong. Thus, they use a Markov Game modeling and investigate the advantages of relaxing it and reasoning about the MTD mechanism over multiple stage attacks.

In contrast to the MTDs for detection surface shifting that are motivated by performance constraints of the underlying network, there is some work that investigates detection surface shifting for the sole purpose of enhancing security. In \cite{colbaugh2012predictability}, the authors use an ensemble of classifiers that can distinguish a mail as spam and switch between them to make it more difficult for the attacker to fool the system. In general, the use of machine learning for anomaly detection \cite{salman2017machine} coupled with the paradigm of MTD for stochastic ensembles \cite{vorobeychik2014optimal,sengupta2018mtdeep} can lead to interesting future research\footnote{In \cite{bhamare2016feasibility}, authors highlight several challenges in the use of supervised machine learning in cloud network settings.}. In these cases, each classifier is a possible action in $A^\mathcal{D}$.

\begin{figure*}
\centering
\begin{tikzpicture}
\begin{scope}[ opacity=0.6]
    \fill[CornflowerBlue!30!white,draw=black] (180:3.5) ellipse (5 and 3.9);
    %\fill[CornflowerBlue!30!white] (180:3) ellipse (6 & 3.6);
    \fill[Goldenrod!30!white,draw=black]  (360:3.5) ellipse (5 and 3.9);
    
 \end{scope}    
     %Refs Constant period switching
    \node at (140:4.9) {\textbf{Constant Period Shifting}};
    \node at (145:4.5) {Zhu et al.~\cite{zhu2013game}};
    \node at (152:4.5) {Manadhata et al.~\cite{manadhata2013game}};
    \node at (159:4.5) {Albanese et al.~\cite{albanese2013moving}};
    \node at (166:4.5) {Carter et al.~\cite{carter2014game}};
    \node at (173:4.5) {Sengupta et al.~\cite{sengupta2017game,sengupta2018moving,senguptageneral}};
    \node at (180:4.5) {Colbaugh et al.~\cite{colbaugh2012predictability}};
    \node at (187:4.5) {Jafarian et al.~\cite{jafarian2012openflow}};
    \node at (194:4.5) {Venkatesan et al.~\cite{venkatesan2016moving}};
    \node at (201:4.5) {Jajodia et al.~\cite{jajodia2018share}};
    \node at (208:4.5) {Thompson et al.~\cite{thompson2014multiple}};
    \node at (215:4.5) {Debroy et al.~\cite{debroy2016frequency}};
    \node at (222:4.55) {Aydeger et al.~\cite{aydeger2016mitigating}};
    \node at (226:4.95) {Algin et al.~\cite{algin2017mitigating}};

    % Hybrid Period Switching
    \node at (0:0) {Clark et al.~\cite{clark2015game}};

    % Ref Variable period switching
    \node at (36:4.6) {\textbf{Variable Period Switching}};
    \node at (28:4.2) {\textbf{$\bullet$ On event switching}};
    \node at (21:4.2) {Van et al.~\cite{van2013flipit}};
    \node at (14:4.2) {Prakash et al.~\cite{prakash2015empirical}};
    \node at (7:4.2) {Zhao et al.~\cite{zhao2017sdn}};
    \node at (0:4.2) {Neti et al.~\cite{neti2012software}};
    \node at (353:4.2) {Chowdhary et al.~\cite{chowdhary2017dynamic}};
    \node at (346:4.2) {Shi et al.~\cite{shi2017chaos}};
    \node at (336:4.2) {\textbf{$\bullet$ Strategic}};
    \node at (329:4.4) {Lei et al.~\cite{lei2017optimal}};
    \node at (322:4.7) {El Mir et al.~\cite{el2016software}};
\end{tikzpicture}
\caption{The time period between two move events is either a fixed interval or decided based on some form of reasoning in the various Moving Target Defenses proposed in the literature.}
\label{fig:when}
\vspace{-1.6em}
\end{figure*}

\subsubsection{\textbf{Prevention Surface Shifting}}\label{prev}
The goal of an MTD that shifts the Prevention Surface is to make the attacker's process costly by introducing uncertainty in their mind about the defense mechanism in place. For example, it becomes difficult for an adversary to realize whether (1) their attack was undetected and thus, went through to the actual system, or (2) was detected and is presently being monitored (in a honey-net setting for example).  
Investigation on MTD techniques for shifting the prevention surface has been scarce, especially in the context of computer networks. We think this is mostly because (1) an administrator can only use these defenses when they are able to identify an attack with high accuracy and (2) identification of attacks itself is a strong assumption. In \cite{chowdhary2017dynamic}, the authors make this assumption and suggest an MTD mechanism that modifies the bandwidth of the network in response to malicious activity. Thus, the configuration space $A^\mathcal{D}$ consists of infinite actions as the bandwidth can take any real value. Similarly, researchers have also considered shifting the time window when replying to a query that may be malicious \cite{clark2015game}. They also consider the deployment of decoy nodes and switching among them in order to hide from an adversary seeking to actively uncover the prevention surface, i.e. the decoy nodes.

\subsubsection{\textbf{Multi-Surface Shifting}}

MTD methods that move multiple surfaces of a underlying network can simply be done by choosing one technology from each of the above sections and combining them together. Yet, there is rarely any work in constructing such hybrid MTDs, i.e. ones that model the shifting of multiple surfaces at the same time. We discuss a few works that try to shift both the exploration surface and the attack surface of a system.

In \cite{venkatesan2016moving}, authors show that constructing a simple proxy-based switching approach is an ineffective defense by introducing a new attack known as the proxy harvesting attack, which explores the surface to collect a set of IPs and then doing a DDoS attack against all of them. To protect against such attacks, they propose an MTD approach that replaces entire proxies followed by the task of remapping the clients to these new proxies. This renders the exploration effort of the attacker useless and at the same time, reduced the attack efficiency of the attacker. As opposed to looking at a particular attack-motivated setting, authors in \cite{zhuang2014towards} formalize the concept of MTD in which they highlight that shifting configuration can include both the attack and the exploration surface but do not go beyond syntactic notions to show how they can actually be done in the case of a real-world system.
%This level of abstraction is either too low for generalization or too high for realization.
In this regard, authors in \cite{lei2017optimal} try to strike a balance and formalize MTD as a \textit{multi-step game} and show some ways in which the exploration surface $ES$ can be shifted or expanded and the attack surface $AS$ can be shifted. Their configuration space, thus, represents the joint space of both the surfaces, i.e. $S = ES \times AS$.

An interesting future direction could be to leverage existing security methods that add capabilities to multiple surfaces and see how MTD can be used in conjunction with them. For example, researchers have inspected the techniques involving  detection of attacks and countermeasure selection in a single framework called NICE \cite{chung2013nice}. Can we leverage this to come with MTD solutions that move both the detection and prevention surface shifting remains an open question? 

We believe the implementation of systems that integrate multiple surface shifting mechanisms under a single MTD mechanism has several challenges. For example, some of the surfaces might render themselves easily to management by a centralized controller like SDN, while others are better suited for movement in a decentralized fashion. As to how these can be combined together is probably not straightforward. We believe that overcoming these challenges will be an interesting research direction in the coming days.

\begin{comment}
\subsection{MTD for Advanced Persistent Threats}
APT attacks are well planned and highly organized in order to increase the probability of attack success. 

The rectangular nodes in the Figure~\ref{fig:mtd-apt} represent the collection of one or more actions, with the rightmost rectangular node being the end goal of the attacker.

The different stages of APT are described below:
\begin{enumerate}
    
 \item \textbf{Reconnaissance -} The beginning of a successful attack starts with the reconnaissance phase. In this stage, the attacker tries to gather a lot of information about the target. Information gathering involves social engineering, reconnaissance, port scanning, service scanning and psychological manipulation of people into accomplishing the goals of attack. Additionally, APT campaigns also query the public repositories such as \textit{WHOIS}, \textit{BGP} looking for the domains and routing information. The attackers try to find the websites with high-risk vulnerabilities, such as \textit{Cross-Site Scripting (XSS)}, \textit{SQL Injection (SQLI)}, \textit{access points}, \textit{virtual hosts, firewalls}, \textit{IDS/IPS}. The reconnaissance is passive in nature and hence difficult to detect. 
    
\item \textbf{Foothold Establishment: }The attackers use the reconnaissance information in order to prepare an attack plan. The information collected can be used to exploit the vulnerabilities found in the target organization's web application, databases, and other software. The details of well-known vulnerabilities can be obtained from vulnerability databases such as \textit{Common Vulnerability and Exposures List (CVE)}, \textit{Open Source Vulnerability Database (OSVDB)}~\cite{ovsdb}, and \textit{NIST National Vulnerability Database (NVD)}~\cite{mell2006common}, where the known and disclosed vulnerabilities have been archived with a vulnerability identifier (e.g. CVE-ID). Additionally, attackers can also find useful information about the vulnerabilities from \textit{dark-web} and \textit{deep-web} forums~\cite{motoyama2011analysis}. Many organizations do not update the current versions of their software even after vulnerability information has been released to maintain business continuity, which allows attackers to exploit the unpatched vulnerabilities.
    

\item \textbf{Lateral Movement/ Stay Undetected: }Once the attacker has gained a foothold into the target environment, he/she can try to move laterally in the target environment and gain access to other sensitive hosts and critical information in the organizational network. The malware used can spread to the neighboring machines in the target environment of the infected system. The goal of this phase is to expand the foothold to other systems in search of the data they want to ex-filtrate. Once the attacker has reached this stage, it is difficult to completely push the attacker out of the environment. Some methods used by attackers during this stage of attack include user account \textit{Password Dumping}, \textit{Hash Dumping}, etc. The harvested credentials facilitate the lateral movement of the attacker and help him in obtaining the restricted information. Tools such as \textit{Windows Credential Editor (WCE)}, \textit{Mimikatz}, \textit{Windows Local Security Authority (LSA)} process are commonly used for dumping credentials.  
    
\item \textbf{Data Ex-filtration: }The attacker tries to ex-filtrate the data collected to their \textit{command and control} $(C\&C)$ center. Most of the intrusion detection and prevention systems do ingress filtering and not \textit{egress filtering}, \textit{data ex-filtration} often goes undetected. 

\item \textbf{Post Ex-filtration: } The goal of the attacker is to maintain persistence in the system for a long duration of time until the funding for attack campaign is finished or the goals of attacking organization/government are achieved. 

\end{enumerate}


As shown in the Figure~\ref{fig:mtd-apt}, different stages of APT (discussed in Section~\ref{aptdef}) propagation can be disrupted using MTD techniques such as exploration and attack surface shifting. The phases 1-3 of APT can be countered by moving system configuration files, ports of the vulnerable applications, host mutation as discussed by Al-Shaer \textit{et al.}~\cite{al2012random}. The information gathered by the attacker during the reconnaissance phase for APT, payloads generated to established foothold and any lateral movement attempts can be delayed by varying the \textit{exploration surface}(\ref{exp}) from time to time. 

The scope of \textit{attack surface shifting} (\ref{att}) in the context of APT spans from phase 2-4 in  Figure~\ref{fig:mtd-apt}. The data ex-filtration, for instance, utilizes fixed open ports to communicate with command and control $C\&C$ center. MTD strategies highlighted by Manadhata \textit{et. al}~\cite{manadhata2013game} shifts set of entry/exit points into the system and set of communication channels. This can lead to continuous connection disruption in the course of APT propagation, and in effect, make long term system exploitation infeasible for the attacker. 

The \textit{detection surface shifting} (\ref{dec}) and \textit{prevention surface shifting} (\ref{prev}) are continuous activities. The network administrator should have continuous monitoring and intrusion detection for identifying malicious activities. As discussed by Sengupta \textit{et al.}~\cite{sengupta2018moving}, detection agents should be shifted continuously and intelligently in order to optimize the network detection rate and performance. 
Chowdhary \textit{et al.}~\cite{chowdhary2017dynamic} utilize an SDN-based rate-limiting mechanism to penalize rogue nodes in the network as a part of prevention surface shifting, which can slow down the data-ex-filtration phase of APT. An attacker who relies on the current view of network information for mounting APT attack will end up spending a significant amount of resources to reach his end goal when a dynamic detection and prevention surface using intelligent MTD is employed. 
\end{comment}

\subsection{When to switch? $\approx$ When to play?}

Having defined the possible configurations that a defender can switch between, the next question to ask is {\em at what point in time does a defender chooses to execute a switch action that changes their present configuration $s$ to another configuration $s'$}? The answer to this question is better given by dividing the works on MTD systems into two broad categories based on how the time window between multiple switch operations is modified-— \emph{Constant Period Switching} (CPS) and \emph{Variable Period Switching} (VPS). We first describe the primary characteristics of these categories and based on it, categorize the different MTDs (see Figure \ref{fig:when}).

In CPS, the MTD systems move from one state to another, mostly in a randomized fashion, always after a constant time period of $T$. This time is heavily dependent on what (surface) is being moved. The bulk of the work in MTD systems reside in this region. On the other hand, in VPS, the time period between one switch can be completely different from the time period of any other switch. We will later see that works in this area can be further sub-divided into three different categories. Although the two classes may seem to be the exact opposite by definition, it is not hard to see that when we talk about multiple surfaces being shifted, it is reasonable to have one surface shift using CPS while the other is shifted via VPS. We end the discussion on `when to switch’ with a discussion of work in this region, which is sparse, opens up exciting avenues for future work in Section~\ref{research}.

%It is easy to notice (see Fig. \ref{fig:when}) that most of the work in the MTD literature has been in the context of CPS, even though variable period switching can render itself in many different ways to the MTD paradigm. In this section, we explore the various classes and highlight how different researches model the aspect of `time period of a deployed configuration' in MTD systems. In cases, where no work has been done so far, we suggest preliminary ideas, which can be opportunities for future work.

\subsubsection{\textbf{Constant Period Switching (CPS)}}

As mentioned, the key idea of these methods is to move the configuration of a system after a constant amount of time. In existing works, this is generally phrased in one of the following ways-— (1) The actions of the defender are played after every time period $T$ (starting at zero) and at that instant, the system moves from one state to another based on the state transition probabilities, or (2) a new configuration is deployed by the defender a time period $T$. However, independent of how it is phrased, they mean the same thing, i.e. to move the surface at time $T$.

A lot of the research works in MTD literature such as \cite{chowdhary2018mtd,sengupta2017game,sengupta2018moving,manadhata2013game,jajodia2018share}, do not explicitly bring up the topic of a time period but inherently assume that the system moves after time $T$.
%Sweeping the conversation on the time period of switching under the rug is common in many cases because researchers often tend to focus on modeling the problem in a theoretical framework while leaving the low-level implementation details of the moving target defenses.
In these works, authors (1) model the problem as a single step game and generalize the solution of this game to multiple stages (not necessarily repeated games), and (2) showcase the problem of \emph{when to switch} as a different one than \emph{how to switch} and only address the latter, forcing the system admin (or defender) to think of both when implementing MTD solutions. Some works, such as \cite{manadhata2013game}, mention the challenge as non-trivial (that comes up during implementation) but do not provide a solution for it.

%we argue that if these MTD systems were deployed with varied period switching, their models might have to take into account more factors in the state space $S$, which might land up changing the answer, if not the methods itself, to their {\em how to switch} question. Although Manadhata mentions this scenario in \cite{manadhata2013game}, he hardly analyzes it. Thus, due to lack of any formal proof as to weather VPS inherently integrates into these mechanisms, we classify them under the heading of CPS.
%\newpage
Some research works explicitly state that the time period is uniform and the equilibrium strategy is played at the start of each stage \cite{zhu2013game, carter2014game,algin2017mitigating}. Note that, some of these works, such as \cite{algin2017mitigating,albanese2013moving}, try different time periods for switching and can only empirically test which works best.
On similar lines, authors in \cite{venkatesan2016moving} address DDoS attacks use the term $\frac{1}{T}$ to denote the frequency of switching while research in \cite{jafarian2012openflow} call $T$ as the mutation interval. Notations like $t_i$ in \cite{colbaugh2012predictability} allow a user to use different time intervals for state $i$ of an MTD system but default to a constant time period in their work.

An interesting question is {\em how long should this time period $T$ be in practice}? In \cite{thompson2014multiple}, the authors varied the time period $T$ from $60-300$ seconds and evaluated based on the likelihood of thwarting a successful exploit, the magnitude of impact for an exploit, and availability of applications to evaluate a good time for rotation operating systems in a network. They noticed that a smaller $T =60s$ was often, good enough to thwart Network Mapping (nmap)~\cite{lyon2009nmap} attacks. Although, OS fingerprinting was accurate in many situations even when $t=60s$, an attacker could not successfully launch an exploit because of the small time window. For $T=300s$, these results were weaker when stacked up against automated attack systems but showed promise when evaluated using manual attacks. In order to allow for fast rotations, the authors set up machines with different OS and after every interval, $T$ redirected traffic to a new OS. To reduce the load on having so many resources available and reduce redundancy, we believe that having at least two systems is necessary to allow for such small time windows, especially when shifting between OSs-- one VMs sets up an environment while the other handles traffic and the role switch in the next time step.

In \cite{debroy2016frequency}, researchers use the knowledge obtained from historical attack data to obtain a cyber attack inter-arrival (CAIA) rate. Then, they create an optimization problem to maximize the time period (denoted at $T_m$) of switching constrained upon the fact that $T_m$ is less than CAIA. On similar lines, authors in \cite{aydeger2016mitigating} have looked at \emph{traceroute}~\cite{padmanabhan2003secure} data between possible source-destination pairs in order to decide a reasonable time period for obfuscating links or mutating routes of ICMP packets on the network. This helps to mitigate crossfire attacks.

An interesting case arises in \cite{al2012random} because the states of this MTD represent a bipartite mapping between hosts and virtual IPs (vIP) and the authors let each edge in the mapping have a separate mutation time. Each host has a mutation rate associated with it (denoted as $R_i$ in their paper) and some hosts belong to a set of High-Frequency Mutation (HFM) set while some cluster of hosts belongs to a Low-Frequency Mutation (LFM) set. To ensure that availability of a host is not impacted, the hosts that exhibit HFM map to two vIPs (one that it was mapped to in the previous round and one to which it is mapped in the present round) for a small time duration compared to the time period of switching. In \cite{albanese2013moving}, the authors also have a local timer, i.e. maintained by each host, whose expiry triggers changes in their vIP. They use ad-hoc messaging to communicate this change to other nodes in the network to enable communication.

\subsubsection{\textbf{Variable Period Switching (VPS)}}

The idea behind this switching strategy, evident from its name, is to have a variable time period for switching from a configuration to another in an MTD environment. For example, if the system transitions through a series of states denoted as $\langle \dots, s, s' \dots \rangle$ and the time for which $s$ (or $s'$) was up is denoted as $t$ (or $t'$), then $t \neq t'$. We believe that doing a VPS along with an MTD mechanism is similar to doing a two-layer MTD where the first layer deals with a meta MTD for shifting the time-surface and then, the second layer MTD is responsible for executing the actual cyber-surface switching. We do not categorize the MTD works under the following sub-classes.

\begin{figure*}
\centering
\begin{tikzpicture}
\begin{scope}[ opacity=0.6]
    \fill[Salmon!30!white,draw=black] (175:3) ellipse (5 and 3);
    \fill[SpringGreen!30!white,draw=black]  (5:3) ellipse (5 and 3);
    
 \end{scope}    
     %Refs Single Stage Games
   \node at (141:4.4)    {\textbf{Single-Stage Modeling}};
   \node at (146:4.2) {Al Mir et al.~\cite{al2012random}};
   \node at (152:4.2) {Jafarian et al.~\cite{jafarian2012openflow}};
   \node at (158:4.2) {Chowdhary et al.~\cite{chowdhary2016sdn,chowdhary2018mtd}};
   \node at (164:4.2) {Zhu et al.~\cite{zhu2013game}};
   \node at (170:4.2) {Manadhata et al.~\cite{manadhata2013game}};
   \node at (176:4.2) {Thompson et al.~\cite{thompson2014multiple}};
   \node at (182:4.2) {Aydeger et al.~\cite{aydeger2016mitigating}}; 
   \node at (188:4.2) {Carter et al.~\cite{carter2014game}};
   \node at (194:4.4) {Sengupta et al.~\cite{vadlamudi2016moving,sengupta2018moving}};
   \node at (200:4.5) {Colbaugh et al.~\cite{colbaugh2012predictability}};
   \node at (205:4.6) {Venkatesan et al.~\cite{venkatesan2016moving}};
   \node at (212:4.4) {Algin et al.~\cite{algin2017mitigating}};

   %Ref Multi-stage game
   
    \node at (36:4.6)    {\textbf{Multi-Stage Modeling}};
    \node at (28:4.2) {Chowdhary et al.~\cite{chowdhary2017dynamic, chowdhary2018adaptive,chowdhary2018markov}};
    \node at (21:4.2) {Manadhata et al.~\cite{manadhata2013game}};
    \node at (14:4.2) {Colbaugh et al.~\cite{colbaugh2012predictability}};
    \node at (7:4.2) {Zhao et al.~\cite{zhao2017sdn}};
    \node at (0:4.2) {Maleki et al.~\cite{maleki2016markov}};
    \node at (353:4.2) {Lei et al.~\cite{lei2017optimal}};
    \node at (346:4.2) {Miehling et al.~\cite{miehling2015optimal}};
    \node at (339:4.2) {Nguyen et al.~\cite{nguyen2018multistage}};
    \node at (332:4.2) {Sengupta et al.~\cite{sengupta2017game,senguptageneral}};
    \node at (325:4.3) {Clark et al.~\cite{clark2015game}};
       
  \end{tikzpicture}
\caption{Game-theoretic modeling for Moving Target Defenses (MTDs), that is necessary for obtaining optimal movement strategies, can be categorized into either single-stage games or multi-stage games. This choice often reflects the type of threat model being considered and the particular system for which the MTD is implemented.}
\label{fig:how}
\vspace{-1.6em}
\end{figure*}

\paragraph{On-event Switching}
Most works that have a variable time period for switching fall under this category. The main idea is that when a particular event occurs, such as detection of an attack, unavailability of a link or a server, the time period is altered and in most cases, a switch action is triggered immediately.
A well-known case study is of the \emph{FlipIt} games \cite{van2013flipit}. The state of the system is represented using a boolean variable that says who is in control of the software environment-- $1/0$ indicate that the defender/attacker has control of the server. The defender gets to perform a move action that alters the configuration of the server only when it is in control of the server. Thus, the time period is dependent on how long an attacker may be in control of the server.

In \cite{zhao2017sdn}, authors update the belief about the sender type (are they malicious?) upon detection of suspicious packets on the network. This belief, in turn, influences the time period of switching. On somewhat similar lines, authors in \cite{neti2012software} have a belief indicating whether a vulnerability is compromised or not. Only beyond a certain threshold, the switch occurs. Other works argue that obtaining belief parameters such as \textit{with what probability is the sender an attacker?} or \textit{With what probability ss the system compromised?} are hard to obtain accurately in cybersecurity settings because they are bases on direct detection of cyber-events. In \cite{chowdhary2017dynamic}, if the admin detects a spike in bandwidth usage of a particular link or sub-net, they change the maximum bandwidth value allocated to that link or the network. Authors in \cite{shi2017chaos} scan open connections routinely and upon detection of unexpected connections, move between MTD configurations to protect the system against port-scanning attacks. 

\paragraph{Strategic}
In order to understand these methods, we first define $T_{\max}$ as the maximum time for which an MTD system can stay in the same configuration. We can now divide the time interval from $0$ to $T_{\max}$ into discrete time intervals and then decide how to pick a $T$, such that $0 \leq T \leq T_{max}$, at which a move occurs.

In \cite{lei2017optimal}, the authors incorporate the time period as a variable in their state $s$. Thus, $s'=(s, T)$ and the \emph{goal} is to find an \emph{optimal strategy} to play in these \emph{new states}. Thus, if the \emph{optimal policy} in state $(s,2)$ dictates the admin to {\em not-switch}, the game moves to the state $(s,3)$ thereby ensuring that the underlying cyber-surface does not shift. On the other hand, a {\em switch} policy transitions the state form $(s,2)$ to $(s',0)$ and the original cyber surface from $s$ to $s'$.
Note that this idea can be extended to other MTD methods that use state information to decide on a movement strategy.
On the other hand, authors in \cite{el2016software} resort to a simple strategy and do not present analysis as to how sub-optimal it is. They set $T_{\max} = \infty$ and based on the \emph{impact} of (known) \emph{vulnerabilities} in the deployed configuration and a threshold, select a $T \in \{0,\dots,\infty\}$. If there are no vulnerabilities whose impact is greater than the predefined threshold, then the system does not move and remains static until a new vulnerability is discovered (either by the defender or an attack).


\paragraph{Hybrid Switching}
Although the idea of having both a CPS and VPS in an MTD mechanism seems counter-intuitive at first, authors in \cite{clark2015game} looks at MTD mechanisms where one layer that shifts the time window of replying to a strategic adversary is done in an \emph{event-based} fashion while the other layer that deploys and moves among decoy nodes to hide from an active adversary is done using a constant time period. This opens up the possibility for works that shift more than one cyber-surface to research into when it is better to select CPS, VPS, or find a good combination of both.

\subsection{How to switch? $\approx$ How to Play?}

In this section, we seek to look at how the policy for a defender who plans to move a particular cyber-surface is decided. As stated before, a few surveys have been solely devoted to analyzing how this question is answered. As all MTD mechanisms can be viewed using the game-theoretic formalism defined above, the survey on the use of game-theoretic methods for network security \cite{roy2010survey} has some overlap with our categorization. As we investigate a subclass of the defense mechanisms, i.e. ones that are based on MTD, we choose to classify our methods based on the following categorization (shown in Figure~\ref{fig:how}).

\subsubsection{\textbf{Single-Stage Modeling}}
%\hl{We can add some scalability concerns as future research work opportunity}
In this section, we investigate how works have tried to infer the \emph{defender's policy} over the action set $A^\mathcal{D}$ by modeling the current state of the MTD system and ignoring history or future considerations. In such cases, the policy obtained for the defender is optimal (or an equilibrium when formulated as a game) if the time horizon for the system is one. 

In \cite{manadhata2013game}, the state of the system can be modified by a pair of actions, one by the defender and one by the attacker at each game stage. The defender's action, in this case, is a mapping $a^\mathcal{D}: F \rightarrow \{enabled,~disabled,~modified,~unchanged\}$ where the set $F$ represents the set of system features. Thus, by applying these actions on a particular feature of the system, it can shift the attack surface. The attacker has the exact opposite action set $A^\mathcal{A}$ and hence, they can {\em re-enable} a port, {\em disable} a functionality etc. The rewards, $R^\mathcal{A}$ and $R^\mathcal{D}$ for the attacker and the defender, are given by weighing the change is system's features $\Delta F$, i.e. the change in the attack surface $\Delta AS$ and the attack surface measurement $\Delta ASM$, as follows.
\[
R^\mathcal{D}(s,a^\mathcal{D},a^\mathcal{A}) = B_1(\Delta F) + B_2(\Delta AS) - C_1(\Delta ASM)
\]
\[
R^\mathcal{A}(s,a^\mathcal{D},a^\mathcal{A}) = B_3(\Delta ASM) - C_2(\Delta AS)
\]
where the $B_i$-s and $C_j$-s are weights defined by security experts of the system. Note that the \emph{cost of a defense} action ($C_1$) and the cost of attack action ($C_2$) are incorporated in the reward. Thus, solving for an equilibrium of this game results in strategies that account for the cost-reward trade-off. The authors find a Subgame Perfect Equilibrium (SPE) in this game and the equilibrium strategy yields the defender's policy.

In \cite{al2012random} and \cite{jafarian2012openflow}, the defender assumes that more the randomness and switching, less the success of the attacker. Thus, they do not need to reason about multiple agents when coming up with action from $A^\mathcal{D}$ in state $s$. A state $s$ is defined by the present set of allocated vIPs to hosts. An action $a \in A^\mathcal{D}$ corresponds to selecting $k$ unused vIPs. They either pick $k$ random vIPs from the free vIPs or use the top-k scanned vIPs based on the assumption that vIPs that have been scanned more have less chance of being scanned again. On these unused $k$ vIPs are selected, they randomly allocate the $k$ present host to them by using a random permutation. 

In \cite{chowdhary2016sdn,chowdhary2018mtd}, the authors explain the game modeling based on a real-world example and compare the effectiveness of reactive based switching and Uniform Random Strategy (URS) respectively. URS, which is found to be more effective, means to pick any of the available action $a \in A^\mathcal{D}$ with probability |$1/A^\mathcal{D}|$. Other works that also use URS as the defender's policy are \cite{thompson2014multiple,aydeger2016mitigating,algin2017mitigating}. In \cite{thompson2014multiple}, given the present deployed OS in state $s$, they consider the remaining OS configurations as defender's potential action in $s$ and play a URS over them. In \cite{aydeger2016mitigating}, given all networking paths from source to destinations, one is picked at random while in \cite{algin2017mitigating}, the authors use to Fisher-Yates shuffling to select a transmission schedule at the start of every round. When no information is available about the attacks and the defender has no preference over the MTD configurations, playing the URS seems a reasonable way to answer the question of {\em how to switch?} Fortunately, more information is often available to the administrator and in such cases, a URS may be sub-optimal.

To address this, in \cite{carter2014game,sengupta2018moving,vadlamudi2016moving,venkatesan2016moving,zhu2013game}, and \cite{wang2019moving}, the authors design a single-stage normal form game in which the defender's action set comprises of switching to any possible MTD configuration and the rewards are defined over the actions sets of both the defender and the attacker. Thus, if the defender chooses to deploy a particular configuration $c \in A^\mathcal{D}$ and the attacker chooses a particular exploit $e \in A^\mathcal{A}$, then the rewards for the players can be read from the normal form game matrix. At equilibrium, a mixed strategy over the defender's actions turns out to be the optimal movement policy. Thus, the defender rolls a dice at the end of each switching period and depending on the result, chooses the next configuration. Note that this is the optimal policy if the game were to be played for just a single time period (time horizon is one). In \cite{wang2019moving}, the authors consider an MTD for IoT scenario and study the characteristics of a Zero-Determinant strategy that results in a dominant strategy for the single-stage game.
%We do not describe the framework of these works in a little more detail to better understand the subtle differences among them.

In \cite{zhu2013game}, the authors assume (1) a zero-sum reward structure, and (2) an threat model in which the attacker is irrational. Thus, the game is played multiple times and in each step, the attacker's play is observed in order to improve the characterization of the attacker's behavior. In order to do so, the utilities of the game are updated after every observation to reflect the rationality of the attacker. After every update, the resulting Nash equilibrium (NE) is played. In \cite{carter2014game}, the authors assume that if the present system is working with an operating system $i$ and the system is made to switch to an operating system $j$, lower the similarity between $i$ and $j$, more secure is the move action from $i$ to $j$. The rewards for choosing action $j \in A^\mathcal{D}$ are defined accordingly and later fine-tuned by simulating the behavior of an adversary. Similar to \cite{zhu2013game}, the NE strategy is chosen to be the defender's policy.

The other works assume that the attacker can observe (before any attack game-play actually beings) and realize the mixed strategy of the defender using maximum likelihood estimates. Thus, authors of \cite{vadlamudi2016moving,sengupta2018moving} concentrate on finding the Stackelberg equilibrium (SE) strategy for the defender. The rewards of this game, for both the $\mathcal{A}$ and $\mathcal{D}$, are obtained using the CVSS metrics of exploits that work in the context of the defender's actions, i.e. the MTD configurations that can be deployed. On similar lines, authors in \cite{venkatesan2016moving} use the notion of SE to obtain defender's strategy to thwart DDoS attacks.

\subsubsection{\textbf{Multi-Stage Modeling}}

Works in these sections reason about (1) the history-- paths that the system has taken, which may be a result of the actions taken by the players, in order to reach the present state, (2) the future-- how the decision in the present state affects the rewards in the future, or (3) both.

In \cite{chowdhary2017dynamic}, similar to the work by \cite{manadhata2013game} in single-stage modeling, the authors discretize the continuous action space of the defender, which represent bandwidth values, to two levels-- high and low. Then they find a meaningful defender strategy over them by ensuring that in a repeated game setting, the advantage that an attacker gained by packet flooding attacks (at some stage in the past) is neutralized by reducing their bandwidth to the low state for $1 \leq x < \infty$ number of game stages.
On similar lines, authors in \cite{colbaugh2012predictability} consider a repeated game setting and analyze the defender's policy against self-learning attackers. They infer that in their case, the optimal policy converges to the URS. Other works like \cite{zhao2017sdn}, also update their belief about an attacker based on observations drawn from multiple plays of the game. This belief is then used to come up with an optimal strategy for the defender.

A set of works in MTD leverage the attack graph of an underlying system to better reason about the sequential process of an attack. In \cite{miehling2015optimal}, the authors model the problem of network intrusion via a Bayesian Attack Graph. The action set for the attacker $A^\mathcal{A}$ includes the probabilistic paths an attacker can take in this graph. Then, the authors map these probabilistic paths with defender's imperfect sensing capabilities to form a Partially Observable Markov decision Process (POMDP)~\cite{russell2016artificial}. Thus, the state and transition of this POMDP are designed to model the attacker's behavior and the optimal policy becomes the defender's strategy in a particular belief state. A shortcoming of this work is that this strategy may be sub-optimal if the \emph{attacker} is (or chooses to) deviate away from the assumptions that inform the POMDP modeling. On the other hand, using a Partially Observable Stochastic Game (POSG)~\cite{hansen2004dynamic} seems unreasonable in terms of scalability for any real-world system.

Authors in \cite{maleki2016markov,chowdhary2018markov,valizadeh2019toward}, and \cite{lei2017optimal} relax the assumption about partial observability and formalize MTD in a Markov Game framework. In \cite{maleki2016markov}, authors consider policies over the defender's action set that comprise of either single or multiple IP hops. Each action results in the defender uniformly selecting the next state give that an attacker samples actions randomly from $A^\mathcal{A}$. They are able to show that multi-element IP hopping actions increases the defender's reward by a greater magnitude compared to static defense strategies. As we will discuss later, the authors do not consider the defender's cost of performing a hop action or the downtime associated with it as apart of the defender's reward function. Thus, the optimal defender policy might not be optimal for real-world multi-layered network attack scenarios.

In contrast, the works \cite{chowdhary2018markov} and \cite{lei2017optimal} incorporates this trade-off in the rewards $R^\mathcal{D}$ and $R^\mathcal{A}$ of the Markov Game, and can thus, generate policies for the defender given each move of the attacker at each step of the game. In \cite{lei2017optimal}, the inclusion of time variable in the state and the trick of including the attack strategies in the state to make solve it as an MDP makes it hard for the solution to seamlessly scale on a large network. In all these works, the impact on performance $C^\mathcal{D}$ is a part of $R^\mathcal{D}$ and often, just a \emph{heuristic idea} as opposed to simulation in a real system that informs these values. The more accurate these measures become, the better is the strategy.
Authors in \cite{sengupta2017game} model both the performance and security concerns in the different way that the above methods. The performance cost is the cost of picking a particular switch while the rewards of the state represent the security costs of picking a particular configuration. Then, they formulate an optimization problem that produces a defender strategy that reduces the cost of switching over two steps (one switch) and maximizes the security over a single step. Although it is known that there may not exist a Markov stationary strategy that is the optimal switching strategy in such cases \cite{vorobeychik2012computing}, the authors in \cite{sengupta2017game} do not discuss how sub-optimal their switching strategies are.

Lastly, authors in \cite{clark2015game} looks at an MTD defense mechanism for deception (obfuscation of the links in order to send attacker to decoy nodes) and model attackers who are actively trying to uncover this deception over a repeated stage interaction. For one problem, they use the Nash equilibrium (NE) while for the other (identifying decoy nodes) they consider the Stackelberg equilibrium (SE) as the defender's strategy. We believe that it is necessary to highlight a shortcoming of the different modeling choices, especially in light of multi-stage attacks and APT scenarios, however optimizing the model and ensuring the scalability is a difficult task, thus we highlight these as possible research opportunities in the Section~\ref{research}.

